Blocks of Lie Superalgebras of Type W(n)

We calculate the blocks of the category of finite-dimensional representations of W(0,n), with n > 2, and show that all are of wild type. As an application, we show that the centre of the universal enveloping algebra is trivial.

==> Makefile <==
name=xxx
inputs=appendix.tex main.tex part1.tex
TEX=elatex

$(name).dvi: main.tex $(inputs);
	$(TEX) main; cp main.dvi $(name).dvi
	cat *.aux > new_aux
	until cmp old_aux new_aux; do \
		cp new_aux old_aux; \
		bibtex main; \
		$(TEX) main; cp main.dvi $(name).dvi; \
		cat *.aux > new_aux; \
	done

$(name).ps:	$(name).dvi;
	dvips -Pcmpsbakoma $(name).dvi -o $(name).ps

dvi:	$(name).dvi;

ps:	$(name).ps;

clean:
	rm -f *.ps *.dvi *.aux *.log old_aux new_aux *.blg *~

